Boosting Isomorphic Model Filtering with Invariants

The enumeration of finite models is very important to the working discrete mathematician (algebra, graph theory, etc) and hence the search for effective methods to do this task is a critical goal in discrete computational mathematics. However, it is hindered by the possible existence of many isomorphic models, which usually only add noise. Typically, they are filtered out {\em a posteriori}, a step that might take a long time just to discard redundant models. This paper proposes a novel approach to split the generated models into mutually non-isomorphic blocks. To do that we use well-designed hand-crafted invariants as well as randomly generated invariants. The blocks are then tackled separately and possibly in parallel. This approach is integrated into Mace4 (the most popular tool among mathematicians) where it shows tremendous speed-ups for a large variety of algebraic structures.

==> scatter_time.data.tex <==
147	55146
242	8860
55	4503
81	3687
137	3612
488	3526
510	3089
183	1972
125	1918
14	1279
20	883
35	560
41	515
116	506
8	410
152	361
10	361
23	327
34	323
125	307
37	268
18	267
79	255
38	191
56	177
58	141
29	138
110	136
99	121
7	112
22	110
80	105
137	104
122	91
74	84
78	83
109	83
21	82
5	79
78	74
86	71
76	66
50	59
51	57
4	56
47	55
50	54
8	52
7	51
22	47
42	41
12	35
39	23
26	23
23	22
24	22
23	21
33	20
29	19
31	18
10	15
23	15
28	12
9	11
10	10
10	10
15	10
20	9
20	9
12	8
6	8
11	8
17	8
13	7
9	7
7	7
11	6
20	6
14	6
15	6
17	6
17	5
5	5
5	5
3	5
5	5
5	5
8	4
12	4
11	4
5	4
8	4
8	4
7	4
7	4
7	4
7	3
5	3
9	3
9	3
9	3
5	3
7	3
4	2
5	2
5	2
4	2
5	2
2	2
4	2
5	2
2	1
1	1
2	1
1	1
2	1
2	1
3	1
2	1
5	0
0	0
4	0
3	0
4	0
4	0
2	0
5	0
1	0
0	0
0	0
0	0
0	0
0	0
0	0
1	0
1	0
0	0
1	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
0	0
574	70000
154	70000



==> scatter_time_basic_vs_random.data.tex <==
5.4	5.4
0.2	0.0
5.5	5.3
7.7	7.3
0.2	0.1
5.0	3.2
487.8	799.1
115.9	110.9
30.7	27.0
26.3	23.4
0.2	0.1
38.8	33.1
10.3	10.2
10.4	10.1
78.2	75.3
1.2	1.2
1.1	1.0
23.0	22.5
33.1	25.0
28.8	27.4
0.0	0.0
4.6	2.5
9.0	4.6
5.3	3.1
7.8	4.6
122.0	116.1
0.7	0.2
15.2	9.1
23.5	23.4
20.0	8.6
79.9	74.1
0.0	0.0
0.0	0.0
19.6	14.4
0.0	0.0
23.1	23.0
0.0	0.0
41.4	40.3
1.2	0.2
99.0	93.3
0.1	0.1
19.6	14.4
0.1	0.1
147.3	858.3
0.4	0.2
0.4	0.2
0.2	0.1
0.1	0.0
136.7	132.9
109.2	103.2
73.6	69.9
16.8	12.2
509.5	513.0
76.3	73.4
56.0	53.9
15.2	14.0
85.6	78.0
28.0	17.4
8.0	5.9
125.0	224.3
110.1	102.2
9.5	6.7
1.6	1.1
55.3	53.4
152.3	152.1
78.1	70.7
11.0	10.5
9.3	4.5
9.3	4.6
11.8	7.4
124.6	123.9
4.5	3.3
49.7	38.6
0.4	0.1
4.6	3.3
6.8	6.3
51.4	44.5
16.8	9.0
8.1	6.6
1.7	1.2
8.2	8.2
13.9	13.7
7.3	5.6
7.3	5.6
79.4	69.9
16.7	9.0
46.8	46.0
58.2	53.9
9.2	9.0
4.7	2.6
6.6	5.2
573.6	576.6
9.3	6.0
5.3	3.8
14.5	9.1
12.0	7.4
182.9	183.3
42.2	40.2
5.4	3.8
50.5	48.6
19.8	19.1
2.0	1.4
4.7	1.0
23.9	22.3
22.2	21.5
21.8	21.2
12.3	6.7
4.9	3.8
3.9	3.9
11.2	5.8
2.0	1.4
0.0	0.0
137.2	123.2
241.7	227.4
7.4	3.9
34.3	32.7
81.3	78.7
20.6	19.8
6.3	4.4
153.7	152.0
3.1	2.0
37.8	36.2
37.1	34.9
10.5	5.8
18.4	17.9
29.1	27.9
34.6	33.1
22.8	21.6
3.5	2.3
4.0	2.3
1.8	1.1
3.7	2.6
3.6	2.4
9.9	9.1
3.5	2.4
12.7	6.6
3.4	2.4
1.3	0.6
4.9	4.3
7.4	6.0
0.1	0.1
0.1	0.1
0.1	0.1
7.5	5.2
4.8	1.3
1.8	1.2
7.3	3.8
1.8	1.2
3.7	3.6
0.2	0.1
2.8	1.7
1.3	0.8
0.0	0.0

